On the unreasonable effectiveness of the post-Newtonian approximation in gravitational physics

The post-Newtonian approximation is a method for solving Einstein's field equations for physical systems in which motions are slow compared to the speed of light and where gravitational fields are weak. Yet it has proven to be remarkably effective in describing certain strong-field, fast-motion systems, including binary pulsars containing dense neutron stars and binary black hole systems inspiraling toward a final merger. The reasons for this effectiveness are largely unknown. When carried to high orders in the post-Newtonian sequence, predictions for the gravitational-wave signal from inspiraling compact binaries will play a key role in gravitational-wave detection by laser-interferometric observatories.

==> arXiv submit/PNAStable.tex <==

\begin{table}[t]
\caption{Current Limits on the PPN Parameters}
{\begin{tabular}{c c l}
\noalign{\smallskip}
\hline
Parameter&Limit&Remarks \\
\hline
$\gamma-1$&$2.3 \times 10^{-5}$&Cassini spacecraft tracking\\
&$4 \times 10^{-4}$&VLBI radio deflection \\
$\beta-1$&$3 \times 10^{-3}$&perihelion of Mercury \\
&$2.3 \times 10^{-4}$&no Nordtvedt effect \\
$\xi$&$10^{-3}$&no anomalous Earth tides\\
$\alpha_1$&$10^{-4}$&no anomalies in Lunar, binary\\
&& pulsar orbits\\
$\alpha_2$&$4 \times 10^{-7}$&alignment of Sun
and ecliptic \\
$\alpha_3$&$2 \times 10^{-20}$
&no pulsar ``self'' accelerations \\
$\zeta_1$&$2 \times 10^{-2}$&combined PPN bounds \\
$\zeta_2$&$4 \times 10^{-5}$&no binary ``self''-accelerations \\
$\zeta_3$&$10^{-8}$&no Lunar ``self''-acceleration \\
$\zeta_4$ &-- &not independent \\
\hline
\end{tabular}}
\label{table:bounds}
\end{table}

